MixEval: Deriving Wisdom of the Crowd from LLM Benchmark Mixtures

Evaluating large language models (LLMs) is challenging. Traditional ground-truth-based benchmarks fail to capture the comprehensiveness and nuance of real-world queries, while LLM-as-judge benchmarks suffer from grading biases and limited query quantity. Both of them may also become contaminated over time. User-facing evaluation, such as Chatbot Arena, provides reliable signals but is costly and slow. In this work, we propose MixEval, a new paradigm for establishing efficient, gold-standard LLM evaluation by strategically mixing off-the-shelf benchmarks. It bridges (1) comprehensive and well-distributed real-world user queries and (2) efficient and fairly-graded ground-truth-based benchmarks, by matching queries mined from the web with similar queries from existing benchmarks. Based on MixEval, we further build MixEval-Hard, which offers more room for model improvement. Our benchmarks' advantages lie in (1) a 0.96 model ranking correlation with Chatbot Arena arising from the highly impartial query distribution and grading mechanism, (2) fast, cheap, and reproducible execution (6% of the time and cost of MMLU), and (3) dynamic evaluation enabled by the rapid and stable data update pipeline. We provide extensive meta-evaluation and analysis for our and existing LLM benchmarks to deepen the community's understanding of LLM evaluation and guide future research directions.

==> 1_Introduction_v1.0.tex <==
\fuzhao{\textbf{What Measures, Improve.} Large Language Models (LLMs)\citep{} have achieved impressive progress over the past few years. Evaluation plays a critical role in the AI community for two reasons: (1) benchmark can provide the early signal to LLM developers to debug and improve the data and model design; (2) benchmark can offer instructions to LLM users to smartly select the model with better cost-effectiveness trade-off. That is, benchmarks provide feedback signals to the whole community including both model developers and users. Then, people optimize the models based on the benchmarks.}

\fuzhao{\textbf{Requirements and Challenges of LLM Benchmarking.} Different from models invented a few years before, LLMs are so strong that we have an expectation of AGI via improving them. Therefore, the first requirement of evaluating LLM is \textbf{comprehensive}. We hope that we are improving everything so that a benchmark with diverse queries and comprehensive coverage is highly desirable. However, benchmarking models comprehensively is expensive and slow. We usually need to collect a huge amount of queries and responses from existing datasets (Static Benchmarks~\citep{}) or human annotators (Dynamic Benchmarks~\citep{}), which are expensive and slow. Additionally, our community is moving very fast and we want to collect the evaluation results to further improve the models as soon as possible.}

\fuzhao{\textbf{\eval: Towards Evaluating LLMs Precisely and Cheaply.} The goal of this work is to build a benchmark being able to help the community move towards AGI precisely and fast. To this end, we design a two-stage pipeline, including (1) detecting queries in the wild; and (2) grounding the mined queries in existing ground-truth-based benchmarks. Specifically, we first introduce an accurate user query retrieval pipeline, including query detection, query filtering, and query classification. In the query detection step, we train open-source LLMs on our self-collected data to uniformly detect queries on Common Crawl splits and obtain 2M user queries. Then, in the query filtering stage, we leverage GPT-4-turbo to filter the non-query sentences. After that, in the query classification stage, we classify the obtained queries by their input and output modalities and retain the text-in-text-out queries for LLM evaluation. To leverage the wild user queries in ground-truth-based evaluation, for each crawled web user query, we match its most similar query from our benchmark pool together with the corresponding ground truth. We name the resulting benchmark as \eval. To increase the separability of models and leave more room for improvement, we extract a hard split from \eval named \eval-Hard.}

% Both the frontier \citep{} and open-source \citep{} LLMs have achieved impressive progress over the past few years. Evaluation score is one of the core objectives to optimize during the development of LLMs, and thus a capable evaluation pipeline lies at the heart of successful model development. Current LLM evaluation approaches can generally be divided into three categories: (1) ground-truth-based evaluation, (2) LLM-as-judge evaluation, and (3) crowdsourcing human-preference-based evaluation. 

% Ground-truth-based evaluation, or closed-ended evaluation, focuses on ranking the outputs of both base and chat LLMs with a set of predefined correct answers. The research community has introduced a variety of ground-truth-based benchmarks \citep{}. It's fast and easy to evaluate LLMs with such benchmarks. Meanwhile, the answer judgment is non-ambiguous and fair due to the close-ended nature of their queries. However, the ground-truth-based benchmarks are often skewed in their topics (as shown in Figure \ref{fig:benchmark_distribution}) and fail to reflect the true distribution of real-world user queries, making it challenging to assess the nuanced and diverse capabilities of LLMs. 

% On the other hand, two other categories of evaluation approaches mainly focus on the open-ended evaluations of chat LLMs. LLM-as-judge evaluation employs frontier models to rank the models' responses to a set of open-ended queries without ground-truths. The queries are either manually designed \citep{zheng2024judging} or from crowdsourcing platforms \citep{}. Due to the high cost of running frontier models as judges, such approaches cannot scale to a certain quantity of user queries that are granular enough to reflect the complexity and diversity of real-world queries and may also skew from the true distribution (as shown in Figure \ref{fig:benchmark_distribution}). Meanwhile, the frontier model judges have shown unfairness in many previous research, such as verbosity bias, position bias, and self-enhancement bias \citep{}. Such bias may introduce unfair model ranking in practical evaluations. As a comparison, Chatbot Arena \citep{} has been considered a capable benchmark for evaluating chat LLMs. Chatbot Arena is a benchmarking platform for LLMs that features anonymous, randomized battles in a crowdsourced setting. Its ample real-world user queries provide a well-rounded and unbiased evaluation of the LLMs, ensuring the correctness and stability of the model rankings. In addition, its real-time nature makes models hard to overfit the benchmark, thus preventing the contamination problem. Nevertheless, it often takes more than 5k human interactions and a few days to get a single stable model score, which is labor-intensive and slow. Meanwhile, the open-ended nature makes it unable to evaluate base models. In addition, a large proportion of open-ended queries, such as writing a traveling plan, may lack a definitive standard to differentiate between good and bad answers \citep{}. As a result, open-ended evaluations are not purely ability-oriented.

%We argue that a capable LLM benchmark should evaluate models in a way that is as close to their real-world use cases as possible. Crowdsourcing approaches, such as Chatbot Arena, meet this criterion by simulating a chat interface to collect real user queries and preferences. However, as mentioned above, such approaches are still problematic. To evaluate models with close settings to real-world use cases while being cheap, fast, fair, and non-ambiguous, we propose WHALE, an approach for building ground-truth-based LLM benchmarks aligned with real-world user queries. We mine user queries from the web and mirror the distribution of wild user queries to existing ground-truth-based LLM benchmarks to improve their data mixture. Specifically, we first introduce an accurate user query retrieval pipeline, including query detection, query filtering, and query classification. In the query detection step, we train open-source LLMs on our self-collected data to uniformly detect queries on Common Crawl splits and obtain 2M user queries. Then, in the query filtering stage, we leverage GPT-4-turbo to filter the non-query sentences. After that, in the query classification stage, we classify the obtained queries by their input and output modalities and retain the text-in-text-out queries for LLM evaluation. To leverage the wild user queries in ground-truth-based evaluation, for each crawled web user query, we match its most similar query from our benchmark pool together with the corresponding ground truth. We name the resulting benchmark as WHALEval. To increase the separability of models and leave more room for improvement, we extract a hard split from WHALEval named WHALEval-HARD.

% We choose to crawl queries from the web for three main reasons: (1) It is more scalable compared to collecting user queries from chat platforms such as Chatbot Arena. (2) The user queries on the web are grounded in a larger user population (all internet users) compared to those from chat platforms, thus being possibly less skewed from the world-level user population. Considering the Chatbot Arena as a counter-example, its user distribution could be skewed to LLM developers or enthusiasts due to its technical attributes. (3) The web queries are of various input and output modalities, which are not available from chat platforms, and we will harness the multi-modal queries in the future evaluations of any-in-any-out models.

% \jinjie{todo: results and findings}
% \begin{itemize}
%     \item 
%     \item 
%     \item 
%     \item 
%     \item 
% \end{itemize}

\fuzhao{\textbf{Why shall we use \eval?} \eval has three important strengths for practitioners: (1) diverse coverage with real-world distribution because our queries are mined from the large-scale web corpus; (2) very fast running due to its small size, \ie XXX queries in total, and human-free evaluation metric; (3) }


\fuzhao{\textbf{Research Contributions}}
\begin{itemize}
    \item We built a pipeline to detect real-world instructions in the wild, which can not only mine queries to build the benchmark but also might provide a scalable solution to collect (almost) infinite real-world instruction following data.
    \item We propose a novel way to use the benchmarks. We show that we can reconstruct the real-world query distribution by smartly mixing the off-the-shelf benchmarks based on the instructions mined on the web.
    \item The resulting benchmark, \ie \eval achieves a significant correlation (0.96) with real-world human preference leaderboard (\ie Chatbot Arena). It is noteworthy that our benchmark is purely built by only XXX queries from the existing benchmarks with ground-truth, so that we can approximate the human preference results very efficiently without large-scale running and dynamic human annotation.
\end{itemize}

==> 1_Introduction_v1.1.tex <==
% \begin{quote}
% \textit{"What gets measured gets improved." --- Peter Drucker }
% \end{quote}
\textbf{That Which is Measured, Improves.}
\vspace{-0.1em}
% \gndelete{Large language models (LLMs) \citep{achiam2023gpt, reid2024gemini, anthropic2024claude, ormazabal2024reka, meta2024llama3} have achieved impressive progress over the past few years.}
Evaluation is essential in the AI community for two main reasons: (1) benchmarks provide early signals to model developers, aiding in debugging and refining data and model design; and (2) benchmarks guide users in selecting suitable models for specific use cases. Thus, benchmarks offer feedback to the entire community, facilitating model optimization.
\vspace{-0.1em}

% \textbf{Requirements and Challenges of LLM Benchmarking.} Unlike models invented a few years ago, LLMs are so powerful that we have expectations of Artificial General Intelligence (AGI) through their improvement. Therefore, the first requirement of evaluating LLMs is \textbf{comprehensiveness}. We hope to improve everything, so a benchmark with diverse queries and comprehensive coverage is highly desirable. However, benchmarking models comprehensively is expensive and slow. We usually need to collect a huge amount of queries and responses from existing datasets (Static Benchmarks~\citep{hendrycks2020measuring, cobbe2021training, rein2023gpqa}) or human annotators (Dynamic Benchmarks~\citep{chiang2024chatbot}), which is costly and time-consuming. Additionally, our community is moving very rapidly, and we want to collect evaluation results to improve models further as quickly as possible. Therefore, the second requirement of LLM evaluation is \textbf{efficiency}. Furthermore, we also want our evaluation pipeline to be precise enough because a more precise evaluation signal can save a lot of time and budget for model evolution. The bias during query collection (query distribution bias as shown in Figure \ref{fig:benchmark_distribution}) and answer judgment (LLM preference bias~\citep{zheng2024judging}) are two main factors that influence the evaluation precision and therefore, the third requirement is \textbf{unbiasedness}. 

\textbf{Requirements and Challenges of LLM Benchmarking.} Unlike the specialized models prevalent until recently, large language models (LLMs) have begun to exhibit powerful general capabilities \citep{achiam2023gpt, reid2024gemini, anthropic2024claude, ormazabal2024reka, meta2024llama3}. Our goal is to enhance all facets of these models to eventually achieve artificial general intelligence (AGI). Thus, a primary requirement for evaluating LLMs is \textbf{comprehensiveness}, but this is hindered by evaluation \textbf{bias}, \textbf{contamination}, and \textbf{efficiency}. Practitioners generally adopt either automatic or human-in-the-loop approaches for comprehensive benchmarking.
Automatic benchmarking typically employs traditional ground-truth-based benchmarks, such as MMLU \citep{hendrycks2020measuring}, which often fail to capture real-world query diversity, or open-ended benchmarks with LLMs as scorers, such as MT-Bench \citep{zheng2024judging}, suffering from preference bias. This query and scoring bias leads to significant deviations from gold-standard evaluation, impeding model development. Additionally, the static nature of automatic benchmarks results in contamination over time, reducing evaluation reliability.
Human-in-the-loop benchmarking, such as Chatbot Arena \citep{chiang2024chatbot}, offers greater impartiality and dynamism but is expensive, slow, and irreproducible.
\vspace{-0.1em}

\textbf{\evalbf: Towards Precise and Efficient Evaluation of LLMs.}
In this work, we aim to establish a benchmark that achie ves the efficiency of ground-truth-based benchmarks while agreeing with real-world user queries and preferences precisely. 
% Because LLMs are intended for real-world deployment and human interaction, aligning evaluation queries with actual user queries is crucial.
To this end, we propose \method, a two-stage benchmark reconstruction pipeline consisting of (1) wild query detection, and (2) grounding existing benchmarks in the mined queries.
We introduce a user query retrieval process, comprising query detection, filtering, and classification. In the detection phase, we train open-source LLMs on self-collected data to detect queries in Common Crawl splits. During filtering, we utilize GPT-4 Turbo to exclude non-query sentences. In classification, we categorize the filtered queries by input and output modalities, retaining text-in-text-out queries for LLM evaluation.
To align benchmark queries with real-world queries, we match each crawled web user query with its most similar query in the benchmark pool and the corresponding ground truth answer. We designate the resulting benchmark as \eval. To improve the benchmark's ability to distinguish strong models, we derive a challenging subset from \eval, termed \evalhard. To mitigate contamination, we periodically update the data points in \eval and \evalhard using our fast, stable pipeline, which performs benchmark mixture with a different batch of wild queries from the same distribution, showing low variance (0.36 Std. on a 0-100 scale) and significant version difference (85\% unique query ratio).
\vspace{-0.1em}

\textbf{Why use \evalbf?} \eval offers five significant advantages for practitioners: (1) \textbf{accurate} model ranking, demonstrated by a 0.96 correlation with Chatbot Arena, (2) \textbf{dynamic} benchmarking enabled by low-effort and stable updating mechanism, (3) \textbf{fast} and \textbf{reproducible} execution, requiring only 6\% the time and cost of MMLU and with no dependence on human input, (4) a \textbf{comprehensive} and \textbf{less biased} query distribution, as it bases queries on a large-scale web corpus, and (5) a \textbf{fair} scoring process, ensured by the ground-truth-based scoring mechanism.

\vspace{-0.1em}
\textbf{Research Contributions}
\vspace{-0.1em}
\begin{itemize}[leftmargin=*]
\item We developed a pipeline for detecting real-world instructions, capable of mining queries to build benchmarks and providing a scalable solution for collecting vast amounts of real-world instruction-following data.
\item We introduced a new way to utilize benchmarks, demonstrating that real-world query distributions can be reconstructed by strategically mixing off-the-shelf benchmarks with web-mined queries.
\item To the best of our knowledge, \eval creates the first ground-truth-based dynamic benchmark with general domain queries, benefiting from a rapid and stable data updating mechanism.
\item The resulting dynamic benchmarks, \ie \eval and \evalhard, exhibit significant correlations (0.93 and 0.96) with real-world human preference leaderboards (\ie Chatbot Arena), showcasing its comprehensiveness, reduced bias, dynamism, and efficiency.
\item We provide an extensive analysis of \eval and other leading LLM benchmarks, delivering detailed insights that enhance the community's understanding of LLM evaluation and guide future research directions.
\end{itemize}


==> 1_Introduction_v1.2.tex <==
% \begin{quote}
% \textit{"What gets measured gets improved." --- Peter Drucker }
% \end{quote}

\textbf{That Which is Measured, Improves.}
% \gndelete{Large language models (LLMs) \citep{achiam2023gpt, reid2024gemini, anthropic2024claude, ormazabal2024reka, meta2024llama3} have achieved impressive progress over the past few years.}
Evaluation is essential in the AI community for two main reasons: (1) benchmarks provide early signals to model developers, aiding in refining data and model design, and (2) benchmarks guide users in selecting suitable models for specific use cases. Therefore, benchmarks offer feedback to the entire community, facilitating model optimization. Consequently, the first requirement for evaluating LLMs is \textbf{impartiality}–we need to optimize the right objectives by ensuring the query and grading impartiality so that the community advances in the right direction.
Unlike the specialized models prevalent until recently, large language models (LLMs) have begun to exhibit powerful general capabilities \citep{achiam2023gpt, reid2024gemini, anthropic2024claude, ormazabal2024reka, meta2024llama3}. We hope to enhance more facets of these models to eventually achieve artificial general intelligence (AGI). Thus, the second requirement is \textbf{comprehensiveness}–holistic queries are desired to assess a wide range of model capabilities.


% \textbf{Requirements and Challenges of LLM Benchmarking.} Unlike models invented a few years ago, LLMs are so powerful that we have expectations of Artificial General Intelligence (AGI) through their improvement. Therefore, the first requirement of evaluating LLMs is \textbf{comprehensiveness}. We hope to improve everything, so a benchmark with diverse queries and comprehensive coverage is highly desirable. However, benchmarking models comprehensively is expensive and slow. We usually need to collect a huge amount of queries and responses from existing datasets (Static Benchmarks~\citep{hendrycks2020measuring, cobbe2021training, rein2023gpqa}) or human annotators (Dynamic Benchmarks~\citep{chiang2024chatbot}), which is costly and time-consuming. Additionally, our community is moving very rapidly, and we want to collect evaluation results to improve models further as quickly as possible. Therefore, the second requirement of LLM evaluation is \textbf{efficiency}. Furthermore, we also want our evaluation pipeline to be precise enough because a more precise evaluation signal can save a lot of time and budget for model evolution. The bias during query collection (query distribution bias as shown in Figure \ref{fig:benchmark_distribution}) and answer judgment (LLM preference bias~\citep{zheng2024judging}) are two main factors that influence the evaluation precision and therefore, the third requirement is \textbf{unbiasedness}. 

\textbf{Large Scale User-facing Evaluation Provides a More Reliable and Holistic Signal.} 
% \textbf{Bias, contamination, and efficiency, three mountains hindering LLM evaluation}. 
Practitioners generally adopt either automatic or user-facing approaches for LLM benchmarking.
Automatic benchmarking typically employs traditional ground-truth-based benchmarks, such as MMLU \citep{hendrycks2020measuring}, which often fail to capture real-world query comprehensiveness and nuance; or employs open-ended benchmarks using LLMs as scorers, such as MT-Bench \citep{zheng2024judging}, suffering from the preference biases of LLM judges. Such biases in query and scoring can lead to significant deviations from gold-standard evaluation, impeding model development. Additionally, the static nature of automatic benchmarks results in contamination over time, reducing evaluation reliability.
Large-scale user-facing benchmarking, such as Chatbot Arena \citep{chiang2024chatbot}, offers greater impartiality, query comprehensiveness, and dynamism due to its large number of real-world user queries and preference judgments. It provides reliable objectives for model development because (1) it judges diverse and complex model responses stably due to the ``wisdom of the crowd'' effect \citep{yi2012wisdom}, where individual judgment noise is averaged out over a large number of samples; and (2) it guides model optimization to meet user needs effectively in practical applications, which is a crucial goal of developing models. However, Chatbot Arena is expensive (Figure \ref{fig:heatmap_arena}), slow, and irreproducible. Moreover, it is not directly accessible for public usage, hindering practitioners from conducting easy and fast model evaluations.

\textbf{\evalbf: Towards Reliable, Holistic, and Efficient LLM Evaluations.}
In this work, we aim to establish a benchmark that achieves the efficiency of ground-truth-based benchmarks while agreeing with real-world user queries and preferences precisely. 
% Because LLMs are intended for real-world deployment and human interaction, aligning evaluation queries with actual user queries is crucial.
To this end, we propose \method, a two-stage benchmark reconstruction pipeline consisting of (1) wild query detection and (2) grounding existing benchmarks in the mined queries.
We introduce an accurate user query retrieval process, comprising query detection, filtering, and classification. In the detection phase, we train open-source LLMs on self-collected data to detect queries in Common Crawl splits. During filtering, we utilize GPT-4 Turbo to exclude non-query sentences. In classification, we categorize the filtered queries by input and output modalities, retaining text-in-text-out queries for LLM evaluation.
To align benchmark queries with real-world queries, we match each crawled web user query with its most similar query in the benchmark pool and the corresponding ground truth answer. We designate the resulting benchmark as \eval. To improve the benchmark's ability to distinguish strong models, we derive a challenging subset from \eval, termed \evalhard. To mitigate contamination, we periodically update the data points in \eval and \evalhard using our fast, stable pipeline, which performs benchmark mixture with a different batch of wild queries from the same distribution, showing low variance (0.36 Std. on a 0-100 scale) and significant version difference (85\% unique query ratio). As shown in Figure \ref{fig:heatmap_arena}, \eval and \evalhard achieve similar model rankings as Chatbot Arena while being far less costly. 

\textbf{Why use \evalbf?} \eval offers five significant advantages for practitioners: (1) \textbf{accurate} model ranking, demonstrated by a 0.96 correlation with Chatbot Arena\footnote{The Chatbot Arena leaderboard is not the sole indicator of real-world human preferences, but it currently serves as one of the gold standards within the community. Therefore, we utilize it as a reliable source of approximation.}, (2) \textbf{fast}, \textbf{cheap} and \textbf{reproducible} execution, requiring only 6\% the time and cost of MMLU and with no dependence on human input, (3) \textbf{dynamic} benchmarking enabled by low-effort and stable updating mechanism, (4) a \textbf{comprehensive} and \textbf{less biased} query distribution, as it bases queries on a large-scale web corpus, and (5) a \textbf{fair} scoring process without preference bias, ensured by its ground-truth-based nature.


\textbf{Research Contributions}

\begin{itemize}[leftmargin=*]
\item We developed a pipeline for detecting real-world instructions, capable of mining queries to build benchmarks and providing a scalable solution for collecting vast amounts of real-world instruction-following data.
\item We introduced a new way to utilize benchmarks, demonstrating that real-world query distributions can be reconstructed by strategically mixing off-the-shelf benchmarks with web-mined queries.
\item To the best of our knowledge, \eval creates the first ground-truth-based dynamic benchmark with general domain queries, benefiting from a rapid and stable data updating mechanism.
\item The resulting dynamic benchmarks, \ie \eval and \evalhard, exhibit significant correlations (0.93 and 0.96) with real-world user preference leaderboards (\ie Chatbot Arena) and showcase comprehensiveness, reduced bias, dynamism, and efficiency.
\item We provide meta-evaluation and extensive analysis for \eval and other leading LLM benchmarks, delivering detailed insights that enhance the community's understanding of LLM evaluation and guide future research directions.
\end{itemize}


==> checklist.tex <==
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We carefully inspected the main claims we made in the abstract and introduction, and ensure that all of them are appropriate.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Limitations are detailed as part of Section \ref{sec:FAQ} in the form of QAs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no theoretical result made.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All implementation details are provided (in Experiment settings and Appendix).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We uploaded the code and data, and will release and periodically update the benchmark data and its related code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We carefully reason our choices in our method and experiment section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide a significance test for the dynamic benchmarking by running 5 versions of 5 random seeds. While for other experiments, it's too expensive to run multiple times.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We specify the hardware we use in the Experiment Settings.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We carefully read and follow the NeurIPS Code of Ethics through out the whole research process.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This research focuses on an improved benchmarking method for LLMs, which does not directly involve significant societal impacts. Its primary influence is within the LLM research community, as detailed in Section \ref{sec:introduction}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Discussed in Section \ref{sec:consideration_web_q_crawl}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We properly cite all the previous work, datasets, or software we use.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We upload and release our data and code with detailed instrutions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No crowdsourcing involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Not available.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}
